Lux: Always-on Visualization Recommendations for Exploratory Dataframe Workflows

Exploratory data science largely happens in computational notebooks with dataframe APIs, such as pandas, that support flexible means to transform, clean, and analyze data. Yet, visually exploring data in dataframes remains tedious, requiring substantial programming effort for visualization and mental effort to determine what analysis to perform next. We propose Lux, an always-on framework for accelerating visual insight discovery in dataframe workflows. When users print a dataframe in their notebooks, Lux recommends visualizations to provide a quick overview of the patterns and trends and suggests promising analysis directions. Lux features a high level language for generating visualizations on demand to encourage rapid visual experimentation with data. We demonstrate that through the use of a careful design and three system optimizations, Lux adds no more than two seconds of overhead on top of pandas for over 98% of datasets in the UCI repository. We evaluate Lux in terms of usability via a controlled first-use study and interviews with early adopters, finding that Lux helps fulfill the needs of data scientists for visualization support within their dataframe workflows. Lux has already been embraced by data science practitioners, with over 3.1k stars on Github.

==> cfg.tex <==
% \begin{equation}
%     \langle Intent\rangle \rightarrow \langle Clause\rangle^* \\
% \end{equation}
% \begin{equation}
%     \begin{split}
%         \langle Clause\rangle &\rightarrow \langle Axis \rangle \\
%         &\rightarrow \langle Filter \rangle 
%     \end{split}
% \end{equation}
% \begin{equation}
%     \langle Axis \rangle \rightarrow \langle attribute \rangle \langle channel \rangle \langle aggregation \rangle \langle bin\_size \rangle
% \end{equation}        
% \begin{equation}
%     \begin{split}
%         \langle attribute \rangle &\rightarrow \textrm{attribute} \\
%         &\rightarrow \textrm{attribute} \cup \langle attribute \rangle\\
%         &\rightarrow \langle wildcard \rangle
%     \end{split}
% \end{equation}
% \begin{equation}
%     \langle wildcard \rangle \rightarrow \textrm{( ? )} \langle constraint\rangle\\
% \end{equation}
% \begin{equation}
%     \langle constraint \rangle \rightarrow \langle data\_model\rangle \langle data\_type\rangle\\
% \end{equation}

\begin{equation}
    \begin{aligned}
        &\langle data\_type\rangle \rightarrow (\textrm{quantitative }| \textrm{ nominal } | \textrm{ ordinal } | \textrm{ temporal } | \textrm{ auto})\\
        &\langle data\_model\rangle \rightarrow (\textrm{dimension }|\textrm{ measure }|\textrm{ auto})\\
    \end{aligned}
\end{equation}

% \begin{equation}
%     \langle Filter \rangle \rightarrow \langle attribute\rangle (=|>|<|\leq|\geq|\neq) \langle value\rangle\\
% \end{equation}

% \begin{equation}
%     \begin{split}
%         \langle value \rangle &\rightarrow \textrm{value} \\
%         &\rightarrow \textrm{value} \cup \langle value \rangle\\
%         &\rightarrow (\textrm{?})
%     \end{split}
% \end{equation}

==> demo_old.tex <==
%!TEX root = main.tex
% \section{Use Case and Design Requirement}
\section{Visual Dataframe Workflows}\label{sec:vdf_workflow}
We first demonstrate 
how always-on visualization support
for dataframes accelerates
exploration and discovery. 
\agp{For each step we should be making sure we
are taking about the interesting aspects of \lux, esp given
that the dataset doesn't teach us anything new.
e.g., \lux notices that the datatype is X and therefore
picks this vis, or \lux recomputes the vis quickly despite
there being a large-scale update to the data, etc.}

\subsection{\lux\label{sec:demo} Example Workfow}
We present a workflow 
of Alice, a data scientist, exploring an 
HR dataset~\cite{ibm_hr}\footnote{The demo video and example notebook can be found in the supplementary materials.}. 
Alice is interested in understanding 
how employee characteristics, 
such as number of years spent working at the company, 
age, and salary rates, might influence attrition. 

\stitle{Always-on dataframe visualization.} 
Alice opens up a Jupyter notebook 
and imports \pandas and \lux. 
Using \pandas's \texttt{read\_csv} command, 
Alice loads the employee dataset 
consisting of 135 columns and 1470 rows. 
To get an overview, Alice 
prints\footnote{We refer to any operations 
that result in a dataframe in 
the output cell of a notebook 
as \textit{printing the dataframe}, 
not the literal `print (df)'.} 
the dataframe \texttt{df} and 
\lux displays 
the default \pandas tabular view, 
as shown in Figure~\ref{fig:print_df} (top). 
By clicking on the toggle button, 
Alice switches to the \lux view 
that displays a set of univariate 
and bivariate visualizations (bottom). 
Visualizations are organized 
into sets called \textit{actions}, 
displayed as tabs along the top of the widget. 
By inspecting the \code{Correlation} action, 
Alice observes several salient patterns 
along with some that poses a sharp triangular pattern. 
This pattern aligns with her intuition 
that total working years must not exceed the employee's age, 
and, similarly, an employee's total working 
years must not exceed their years at a given company. 
She also examines the other tabs of the \lux widget, 
which show the \code{Distribution} of quantitative attributes 
and the \code{Occurrence} of various categorical attributes. 
\begin{figure}[h!]
    \includegraphics[width=\linewidth]{fig/demo/1-print_df.pdf}
    \caption{By printing out the dataframe, 
    the default \pandas tabular view 
    is displayed (orange) 
    and users can toggle to browse 
    through visualizations recommended by \lux.}
    \label{fig:print_df}
\end{figure}
\stitle{Steering analysis with intent.} 
Next, Alice wants to investigate factors 
that influence employee attrition. 
As shown in Figure~\ref{fig:set_intent}, 
she programmatically specifies her analysis \textit{intent} 
to \lux as: \texttt{df.intent = ["Attrition"]}. 
On printing the dataframe again, 
\lux employs the specified analysis intent 
to steer the recommendations towards what 
Alice might be interested in. 
On the left, Alice sees the visualization 
based on her specified intent, 
showing that $\approx15$\% of
the employees leave the company. \todo{[leave or have left? when do they leave?]}
On the right, Alice sees two sets of 
recommendations that add an additional attribute (\code{Enhance}) 
or add an additional filter (\code{Filter}) 
to her intent \text{Attrition}. 
By looking at the bar chart in the \code{Enhance} action 
(chart with the orange box in Figure~\ref{fig:set_intent}), 
she learns that employees that leave 
typically spent less time 
in their working life at the Company 
than their counterparts by about four years. 
Alice wants to understand whether 
the lower number of years at the company 
can be attributed to younger employees who
had a lower number of working years overall, 
or whether these were middle-aged employees 
who truly spent fewer years at the company. 
To do so, she derives a new column 
that captures the percentage of 
the employee's working years 
have they spent at the company. 
% \marti{explain this reasoning more; why does she do this? first state a higher level motivation such as: has the employee spent most of their working life at this company, or are they a new hire, or something in between?  This reduces the work for the reader following your example.} \doris{added extra description and also reference figure.}
% \marti{I don't understand this wording; it seems like it's saying the left is relevant to Intent and the right is relevant to Intent.  These all seems to be recommendations.  What is the difference between them? }\doris{reworded for clarity} 

\begin{figure}[h!]
    \vspace{-10pt}
    \includegraphics[width=\linewidth]{fig/demo/2-set_intent}
    \vspace{-10pt}
    \caption{Alice sets the intent based on the attribute \texttt{Attrition} and \lux displays visualizations that are related to the intent.}
    \label{fig:set_intent}
    \vspace{-20pt}
\end{figure}
She prints out and inspects the 
computed percentages, 
corresponding to a 1-D Series 
object\footnote{\url{https://pandas.pydata.org/pandas-docs/stable/reference/api/pandas.Series.html}}. 
The Series visualization not only 
enables her to quickly verify that the 
data lies between 0 and 1, 
but also reveals that there is a 
large group of employees who have 
spent almost all of their working life at this company. 
She creates a new column \texttt{\%WorkingYearsAtCompany} to capture this metric.
% \marti{Why is this a surprise?  I expected this when I wrote the comment above; I hadn't looked at the distribution yet.  Is Alice  very naive about HR data or does she have some reason for this assumption?  If so, this needs to be built into the start of the case study.}
\begin{figure}[h!]
    \includegraphics[width=0.9\linewidth]{fig/demo/3-series_vis}
    \vspace{-10pt}
    \caption{Series visualization enables quick inspection of the data present in the column.}
    \label{fig:series_vis}
    \vspace{-15pt}

\end{figure}
\stitle{Quick-and-dirty experimentation with \vis and \vislist:}  
So far, we have demonstrated 
how always-on visualizations 
for dataframes and series 
can enrich an exploration workflow. 
Say Alice now has a specific hypothesis that 
she wants to investigate---are there 
any differences in 
percentage of working years at the company 
for young employees compared to senior employees?. 
She generates a \vis 
showing the relationship 
between \texttt{Age} 
and \texttt{\%WorkingYearsAtCompany} (Figure~\ref{fig:quick_vis} left). 
However, the trend is unclear.  
As a result, she decides to bin 
the \texttt{Age} variable into Booleans 
based on whether the employee 
is above or below 
the average employee age, called \texttt{Senior}. 
She then creates a \vis object 
involving the two attributes; 
\lux automatically displays 
a bar chart showing that senior employees 
have a smaller percentage 
of working years at the company (Figure~\ref{fig:quick_vis} right). 
\begin{figure}[h!]
\vspace{-10pt}
    \includegraphics[width=\linewidth]{fig/demo/4-quick_vis}
\vspace{-15pt}
    \caption{Creating \vis is a quick way to plot visualizations and investigate specific hypotheses.}
    \label{fig:quick_vis}
\vspace{-10pt}
\end{figure}
% By printing out the list of columns in the dataframes, she notices how there are several attributes related to hourly, daily, and monthly compensation and investigates whether senior or younger employees gets paid more. By generating a \vislist consisting of the compensation-related attributes and the \texttt{Senior} indicator. She skims through the list of visualizations returned by \lux and finds that the differences are not significant.
She then groups the dataframe 
by the \texttt{Senior} 
indicator to investigate 
other differences across 
senior or young employees; 
\lux displays the 
aggregated measures as 
a list of visualizations (Figure~\ref{fig:quick_vislist}). 
She skims through the list of visualizations 
and finds that the differences 
are not significant across age groups 
for most attributes 
except for the ones that have 
a clear relationship with experience, 
such as job level, monthly income, 
and the number of past companies. 
The programmatic generation of \vis 
and \vislist provides a quick and dirty 
way for Alice to ask specific questions about the dataframe.
\begin{figure}[h!]
\vspace{-5pt}
    \includegraphics[width=\linewidth]{fig/demo/5-quick_vislist.png}
\vspace{-15pt}
    \caption{A \vislist for visualizations based on the \texttt{Senior} indicator.}
    \label{fig:quick_vislist}
\vspace{-10pt}
\end{figure}
\stitle{Exporting visualization code:} 
After reviewing the age-related differences, 
Alice proceeds with her analysis 
of employee attrition by printing 
out the dataframes again. 
Note that \lux retains the analysis intent 
with the updated dataframe. 
Alice learns that employees who 
live further away from work 
tend to have higher rates of attrition. \agp{How does she learn this?} 
She clicks on the visualization in the \lux widget 
and the \includegraphics[height=1em,trim=0 10 0 0]{fig/demo/6-export-btn} button to export the visualization from the widget to a \vis object in the notebook. 
The exported \vis can be accessed via the \texttt{df.exported} property and further printed as code. By copy and pasting the visualization code into a different cell, Alice tweaks the plotting style before sharing the finding with her colleagues. 
%\marti{Does this deserve its own figure?  If so, make the code aspects of the export clearer.}\doris{This is probably not necessary, I've removed this figure.}
% \begin{figure}[h!]
%     \includegraphics[width=\linewidth]{fig/demo/6-export.pdf}
%     \caption{User can quickly export visualizations from the widget as code to edit and share.}
%     \label{fig:export}
% \end{figure}

%even with updated dataframe now contains the two additionally-derived columns. 

% Outline
% - import lux, load in dataset
% - print df, toggle 
% - data cleaning + transform, then revisualize (keep same intent)
% - specify intent steer recommendations
% - demonstrate series and index visualizations
% - export vis, to code, to HTML report
% - create vis/vislist explicitly
% - missing index vis demo but covered in later sections


==> design_motivation.tex <==
\section{Supporting a Visual Dataframe Workflow}
The design motivation for Lux came from our prior experience with users of visual querying and recommendation systems~\cite{zvcell,Lee2019VAST}, as well as the challenges that we observed with exploratory visualizations in computational notebooks. 
\par In a formative design study, we analyzed a corpus of publicly-available notebooks to better understand current visual data exploration practices in computational notebooks. We inspected the notebooks that made use of \pandas and \mpl with a focus on cells that led to visualization outputs. %The initial focus of our analyses was to better understand the strategies, patterns in the analytical decisions~\cite{Liu2020-paths} that led users to exploratory insights. As a result, w
    \par We found a surprising number of notebooks that shared a similiar structure for exploratory visualizations. These workflows apply a series of \textit{data processing} operations to wrangle the dataframe into a form that was amenable to visualize. This is often followed by a set of highly-templated \textit{visualization specification} code copy-and-pasted and reused across the notebook, echoing similar finding in ~\cite{copypastenotebook}. Not only is there a high formulation cost associated with writing ``glue code'' to go from dataframes to visualizations~\cite{Wang_Viser2020,alspaugh2019}, users have to context-switch between thinking at the level of data operations \tr{(e.g., how to reshape data? what aggregation or filter to apply?)} and thinking about visual elements \tr{(e.g., what graphical marks to chose? what channel to encode attribute?)}. \tr{These barriers often hinder exploratory visualizations and as a result, users often only visualize during ``\textit{isolated late stages of [their] workflow}''~\cite{Batch2018,Kandel2012Interview}, rather than visualizing whenever they want.}%In manual df, data operations are isolated from vis operations. Vis is post-hoc rather than in-situ. 
    \par These challenges inspired us to design an always-on visualization framework that seamlessly integrates with a dataframe-based workflow. We envisioned a natural, intuitive experience that ``looks and feels'' like a \pandas dataframe, but with additional visual affordances. Next, we outline the set of design requirements based on our formative experience with early-users.
    \subsection{Design requirements}
    \stitle{D1: Always-on, immediate visual feedback}%perspective?
    \npar \tr{Printing the tabular view of the dataframe is one of the most common ways that users inspect and validate the dataframe against their mental models of an intended operation~\cite{modin-vision}. }While tables are an effective form of visualization\tr{ for understanding dataframe structure and schema}, many exploration tasks are more amenable with chart-based visualizations. In order to encourage ``flow'' and minimize visualization overhead, our goal is to provide a visual representation of the dataframe at any point in user's analysis workflow. 
    %Moreover, to avoid information overload, effective visual feedback should be relevant to the user's analysis context.
    %print and get vis right away (different from generation of report, pandas-profiling) 
    \stitle{D2: Preserve dataframe functionality as-is}
    \npar %The success of \pandas as a dataframe implementation is often attributed to its comphrensive array of convenient APIs, spanning from relational operators to advanced statistical functions. 
    To preserve the comphrensive array of convenient APIs offered by dataframes, we aimed to natively support any possible operations that a user could perform with their \pandas dataframes. This design requirement minimizes the need for importing and exporting data to and from visual tools (common in the case of visualization GUIs) and the need for learning a new API (common in the case of visualization libraries). 
    \stitle{D3: Keep underlying dataframe immutable}
    \npar Dataframes often serve as an intermediate data structure for data scientists to load, clean, and transform their data. As a result, dataframes can often be ill-formatted in a way that is not amenable to visualizations. To allow users to effectively operate on their data, it is crucial that the system provides users with the \textit{unmodified}, \textit{consistent} state of the dataframe. In other words, the system should not attempt to modify and change the user's dataframe in the process of visualization to maintain WYSIWYG behavior. This design requirement motivates the decoupling between dataframe content and the views built on top of it, described next.
    % Maintain user control WYSIWYG
    % One example of this is handling missing values, or when dataframes contains mixed datatypes (a common issue when loading in spreadsheets).

==> design_requirements.tex <==
\subsection{Design Requirements}
The design motivation for Lux came from our prior experience with users of visual querying and recommendation systems~\cite{zvcell,Lee2019VAST}, as well as the challenges with exploratory visualizations in computational notebooks~\cite{Wang_Viser2020,copypastenotebook,nbsurvey}. 
\dtc{How these requirements are related to challenges? I did not fully get the second one.}\doris{I don't think the requirements translate to challenges well in a 1:1 manner. I'm wondering if we should just remove this entire subsection alltogether.}
    \stitle{D1: Always-on, immediate visual feedback}%perspective?
    \npar \tr{Printing the tabular view of the dataframe is one of the most common ways that users inspect and validate the dataframe against their mental models of an intended operation~\cite{modin-vision}. }While tables are an effective form of visualization\tr{ for understanding dataframe structure and schema}, many exploration tasks are more amenable with chart-based visualizations. In order to encourage ``flow'' and minimize visualization overhead, our goal is to provide a visual representation of the dataframe at any point in user's analysis workflow. 
    %Moreover, to avoid information overload, effective visual feedback should be relevant to the user's analysis context.
    %print and get vis right away (different from generation of report, pandas-profiling) 
    \stitle{D2: Preserve dataframe functionality as-is}
    \npar %The success of \pandas as a dataframe implementation is often attributed to its comphrensive array of convenient APIs, spanning from relational operators to advanced statistical functions. 
    To preserve the comphrensive array of convenient APIs offered by dataframes, we aimed to natively support any possible operations that a user could perform with their \pandas dataframes. This design requirement minimizes the need for importing and exporting data to and from visual tools (common in the case of visualization GUIs) and the need for learning a new API (common in the case of visualization libraries). 
    \stitle{D3: Keep underlying dataframe immutable}
    \npar Dataframes often serve as an intermediate data structure for data scientists to load, clean, and transform their data. As a result, dataframes can often be ill-formatted in a way that is not amenable to visualizations. To allow users to effectively operate on their data, it is crucial that the system provides users with the \textit{unmodified}, \textit{consistent} state of the dataframe. In other words, the system should not attempt to modify and change the user's dataframe in the process of visualization to maintain what-you-see-is-what-you-get (WYSIWYG) behavior. This design requirement motivates the decoupling between dataframe content and the views built on top of it, described next.
    % Maintain user control WYSIWYG
    % One example of this is handling missing values, or when dataframes contains mixed datatypes (a common issue when loading in spreadsheets).


==> limitation.tex <==
\subsection{Limitations}
Intent language does not support interactive vis, e.g. cross filter, brushing-and-linking, since the goal was to support more exploratory ``quick-and-dirty'' visualization use cases, support for richer interaction may be future work.
The intent language has limited support for task-oriented goals such as compare differences or detect outliers.
The intent language is not designed to support inquiries across multiple dataframes. The current way to support multiple tables is through a physical join (in the case of pandas), or a virtual view joining multiple tables (in the case of SQL).

==> modin-rebuttal.tex <==
%!TEX root = modin-vision.tex

\begin{center}
{\LARGE \bf Summary for Revised Paper ``Towards Scalable Dataframe Systems''}
\end{center}

We thank the reviewers and meta-reviewer for their detailed 
and insightful feedback, and for giving us the opportunity 
to address their feedback in a revision.  
We have prepared a new version of the paper based on their suggestions, 
with updates to every section. 
In brief, the changes made include:

%\begin{compactenum}
%\item 
\smallskip
\noindent {\bf \em A. New section on challenges 
stemming from the dataframe data model and algebra.} 
We have rewritten 
Section~\ref{sec:datamodel} to center around the
unique characteristics of the dataframe data model
and algebra, 
and framed our research challenges with respect
to these characteristics.
These characteristics include
lazy typing and flexible schema,
the equivalence between rows and columns and 
data and metadata, as well as the centrality of ordering. 
The entirety of this section was rewritten
to address the concerns of the Reviewers and Metareviewer.

\smallskip
\noindent {\bf \em B. New section on challenges
stemming from the use of dataframes in data exploration.} 
We have likewise rewritten 
Section~\ref{sec:interactivity} to focus on the unique
challenges presented by the interactive approach 
for working with dataframes during data exploration. 
In particular, the new discussion centers
around the challenges associated with supporting
the incremental composition of dataframe expressions,
the need for inspection of intermediate results
for debugging and feedback,
and the trial-and-error nature of dataframe-based 
exploration.

\smallskip
\noindent {\bf \em C. Reorganization and reframing of paper grounded
in our experiences with \modin.}
Recognizing that reviewers were unclear about the structure
of the paper and what constituted the visionary part,
we reorganized the paper to move the discussion about our existing system
\modin first.
Specifically, we highlight early on
how our experience thus far in developing \modin informed our vision and
research agenda for the development of (a) an clean formalism
for the dataframe algebra, and (b) an optimized system for implementing
this formalism. 
We also significantly trimmed our discussion of \modin
and its optimizations.
These changes affect
the overall tone of the entire paper 
but are particularly evident
in the new Section~\ref{sec:modin}.

\smallskip
\noindent {\bf \em D. Centering the discussion of challenges around differences
between dataframes and relations.}
In addition to our changes in Section~\ref{sec:datamodel}
and Section~\ref{sec:interactivity},
where we focus on novel challenges that arise in dataframe
systems when contrasted with relational databases,
we also updated the rest of the paper to reflect this tone.
In particular, large parts of Section~\ref{sec:intro} were rewritten
to describe the novel challenges with the dataframe data model
and algebra as well as novel challenges in how dataframes
are manipulated during data exploration workflows. 


\smallskip
\noindent {\bf \em E. De-emphasis and removal of non-visionary aspects.}
In addition to removing content in Section~\ref{sec:modin}, 
we have also made our example in Section~\ref{sec:usecase}
much more concise,
as they both did not add to the visionary content of the paper.
We have also removed or rewritten 
substantial portions of text 
in Section~\ref{sec:definitions} around 
obvious rewriting rules (leaving as-is a single case study
centered on pivot), the comparisons between the dataframe 
data model and other data models, as well as
extensions to the dataframe data model.
Instead, we used that space to augment Sections~\ref{sec:datamodel} and \ref{sec:interactivity} with new visionary content.


\smallskip
\noindent {\bf \em F. Other significant writing changes.} 
We have made considerable changes to the text 
of the paper to improve its overall readability. 
Specifically, we have focused on making the paper 
more clear, formal, and concise. 
We have rerun an experiment to verify that
a spike was indeed due to experimental variance.
Finally, we have also improved presentation by replotting figures, 
making our notation consistent, and fixing typographical errors.

\smallskip
The changes in the paper are highlighted in \rebuttal{\bf purple}. 
Unfortunately,
due to the new additions, this meant that our paper ended up being longer than we could fit in the 12+4 pages;
additional details  can be found in our extended technical report~\cite{petersohn2020towards}.
%\end{compactenum}
We address the specific points raised in each of the individual reviews below, starting with the meta-review.


\subsection*{Metareview}
\com{(M1) 
The description of the existing system should be reduced and rephrased
to be more of a technical background rather than 
sounding like a research paper.
}

We have substantially reduced the amount of
detail in each of 
Sections~\ref{sec:usecase}, \ref{sec:modin}, 
and \ref{sec:definitions}, and 
only kept details
that are pertinent to the vision components of the paper. 
We now describe in detail what was
removed or revised.

In Section~\ref{sec:usecase}, 
we removed portions
that were self-explanatory or easily understood. 
We also replotted Figure~\ref{fig:example} 
to take up less space. 
Descriptions of how users 
interact with a dataframe system 
were moved to later sections 
when describing the motivations for 
improving certain interaction modalities.

In Section~\ref{sec:modin}, we substantially 
reduced the amount of detail on our current implementation
of \modin.
Recognizing the purpose of this section
is to describe our experience with dataframes
thus far, and to use that to 
set the stage for our future research
agenda, we moved this section
to right after Section~\ref{sec:usecase}
as our prior work.
We entirely removed any architectural
descriptions about \modin as they are not relevant
for our vision. 
Since the techniques underlying \modin 
thus far are straightforward, we
made their description much more concise.
Since there was also 
some confusion about what had been implemented 
and what was future work, we
also cleared that up by making 
Section~\ref{sec:modin} the ``already implemented''
component and making 
latter sections more vision-oriented to convey
that those are indeed future work. 

In Section~\ref{sec:definitions}, we have made substantial
changes to all subsections.
We removed much of the detailed
discussion on the finer points of the described
data model in Section~\ref{sec:dataframedef}.
Some of this detail was moved
to Section~\ref{sec:datamodel} to motivate 
some of the research challenges in dataframes, 
but many details were removed entirely from the
paper if they did not add to the overall vision.
We also replaced some lengthy text with two compact
tables. 
We entirely removed the workflow definitions part,
choosing to introduce some of these terms 
as needed later on.
In Section~\ref{sec:df-algebra}, 
we made significant cuts to the explanation of
the operators. 
Since this paper does not try to argue
minimality, we use
these operators more as a frame of reference 
to describe the new challenges in efficiently
processing dataframes as opposed to providing
formal definitions. 
We only kept the components that tie 
directly to later sections of the paper 
where our future research problems are described. 
We have revised Section~\ref{sec:algebra-example}
to only convey one single case study on \code{pivot}
as opposed to many straightforward examples
of rewriting of \pandas API operators into
the dataframe algebra.
(We also enhanced this case study to add more
detail, along with a new figure.)
Former Section 3.5 (now would be 4.5) was entirely
removed, since the extensions to the data model
does not add much to the vision portion of the paper.


While we have cut back substantially in all of
Sections~\ref{sec:usecase}, \ref{sec:modin}, 
and \ref{sec:definitions},
further cuts would hurt understanding 
for database readers. 
Specifically, we believe an important contribution 
of this paper is to provide some background into 
dataframes and their characteristics.  
One of our reviewers remarked that they were skeptical of
any difference between dataframes and databases before they read this paper,
but this background was effective in convincing them 
that they are distinct artifacts
and will require a new body of research.


\com{(M2) 
The integration between the technical background and the vision needs to be improved.
Specifically, the vision focuses on the more general problems in data exploration
and does not focus on how these problems are different in dataframes
(as compared to relational settings).
}

\com{AND}
% We combine our comments for (M2) and (M3) to avoid repetition and
% for ease of review.

\com{(M3) 
The identification of the unique challenges of dataframes needs to be better.
Additionally, the challenges of relational systems which dataframes exacerbate
and that which dataframes lessen. 
}

To highlight how the discussed 
challenges are specific to dataframes,
we have significantly restructured the paper to provide
a more familiar flow
and have substantially revamped
Sections~\ref{sec:datamodel} and \ref{sec:interactivity}
taking the reviewer comments into account.

Specifically, for Section~\ref{sec:datamodel},
we had originally anchored our discussion around
``layers'' of a database system architecture 
to provide a familiar point of entry for a VLDB audience.
Likewise, for Section~\ref{sec:interactivity},
we had originally organized our proposed directions 
around ideas (many of them stemming from general
data exploration) as opposed to unique dataframe aspects.
We also focused too much on solutions rather than the underlying problems and why they are interesting
and unique.
After reading the reviews, 
however, we realized that this was not an optimal approach
for conveying our vision for scalable dataframe systems. 

As such,
we have now focused these sections around 
unique challenges in the dataframe
data model and algebra (Section~\ref{sec:datamodel}) 
and in how dataframes are manipulated over
the course of a user exploration session
(Section~\ref{sec:interactivity}).
When describing these challenges, we focused
on the key differences between operating on dataframes
and on relations. 
%We have also added a new section,
%Section~\ref{sec:algebra-challenges}, to discuss the challenges specific to
%the new algebra and our vision on how systems might solve some of those problems.
Prior to these sections, we 
set the stage for our research vision in the
substantially revised Section~\ref{sec:modin}
which describes what has been implemented,
and how that informs our future agenda.
We now explain the changes to Sections~\ref{sec:datamodel} and ~\ref{sec:interactivity}
in detail.

In Section~\ref{sec:datamodel}, we organize
our discussion around various unique properties
of dataframes, including flexible schema, lazy typing,
row-column equivalence (thanks to operators such as transpose), data-metadata equivalence (thanks to the presence of 
row and column labels
and operators that allow labels to become part of data),
and the centrality of order for both rows and columns. 
We ground this discussion by drawing on prior work in the
relational database community, and discuss why those
techniques would not apply to dataframes without violating
key dataframe properties. Grounding
the discussion in this manner helps us contrast the future
work needed to develop dataframe systems with existing work 
on relational databases.

% \agp{There is some text following this that I don't like 
% that elaborates on the previous. We can possibly
% omit it and leave it as it is above. Or revise it as time permits.}
% \devin{See above}
% \done{
% We first focus
% on the challenges of supporting flexible schemata, which is a particularly
% salient property for dataframes. Re: lazy typing, we describe when and how the schema 
% induction function $S$---a costly operation---should be invoked
% to induce the schema, 
% and how its invocation can be avoided if possible.
% We also discuss how difficult certain optimizations, like memory layout and
% compression, will be difficult in dataframes and require new techniques which
% will be developed as dataframes are researched.
% We then
% describe another unique property of dataframes, order as a first-class citizen,
% and the challenges involved in supporting order. We discuss works in relational
% algebra that may partially apply and certain cases where novel approaches will
% be needed. We discuss different hypothetical memory layouts for presenting
% data as ``ordered'' without placing physical requirements on ordering the
% data. We also discuss challenges and potential solutions in the area of query
% optimization when users must be presented an ordered view.
% }
% \agp{end text that may be deleted/revised}


%\done{
%\stitle{Section~\ref{sec:algebra-challenges}}. Many points in the algebra section
%were discussions on the challenges in supporting the algebra, but this structure was
%not condusive to the vision structure. Instead, we have created a new subsection and
%included the discussion around the challenges in supporting
%specific operators. We have expanded on the challenges and included
%our vision of potential pitfalls of certain approached moving forward.
%}

In Section~\ref{sec:interactivity},
we have centered our research challenges around the unique
ways in with dataframes play a role in data exploration.
Specifically, dataframes are usually manipulated interactively
over the course of a long-running user session,
with dataframe queries composed incrementally as individual \stmts,
a small number of operators at a time,
with subsequent invocations building on previous ones. 
Users often revisit previous steps in their exploration,
trying out different exploration strategies in a trial-and-error fashion.
They also inspect intermediate results often with 
an eye towards debugging and validation.
These characteristics are unique to how dataframes
are manipulated across data exploration sessions
typically performed in an interactive environment
such computational notebooks.




% \done{
% This feedback was addressed while resolving (M2).
% }


\subsection*{Reviewer 1}
\com{(A1) It is unclear as to which parts are the technical details
that are currently implemented in the system (which are less suited for a vision paper)
and which parts are the novel visionary contributions of the paper.
}

This feedback was addressed while resolving (M2/M3).


\com{(A2) 
It would be nice to see more discussion 
on the semantics of the group-by (resp. window) operator.
}

We thank the reviewer for this suggestion. We agree that
the semantics of dataframe \code{GROUPBY} and \code{WINDOW} deserve
special attention, particularly the ways in which they
deviate from their SQL/relational algebra counterparts. 
In particular, the fact that dataframes can support
composite types per cell
means that the dataframe algebra can use a broader class of aggregation
functions, not restricted to those that result in a single atomic value. This behavior
is also reflected in \pandas' \code{groupby} operator.
We have added additional
discussion in Section~\ref{sec:df-algebra}, highlighting how certain
functionality can be expressed more elegantly using the dataframe
variants of these primitives.
% , while additionally admitting challenges
% for query planning and optimization.

%\agp{We need to do something for this. A few lines
%in the algebra section will do.}
%\devin{Do we? Can't we say that there are no real dataframe
%challenges outside of the order? We discuss the Window op there}
%\done{
%To keep the vision central to the paper, 
%we have added an entire section to the paper on our vision
%of the challenges related to the algebra and operator set that is 
%exposed by \pandas and other dataframe implementations, 
%Section~\ref{sec:algebra-challenges}. The new section serves as the discussion
%for the vision of optimization based on query planning and optimization
%given a new set of algebra operators.
%Specifically, in \pandas, the semantics are a column-wise groupby followed
%by some operator. There is an intermediate object created by
%\code{df.groupby} calls in \pandas, which can be reused. We can express this
%semantic difference in the algebra with a \code{GROUPBY} on each column,
%followed by the aggregation.
%}

% \todo{
% \stitle{Alternative.}
% We added a discussion around the challenges of the groupby and
% window operators in dataframes in Section~\ref{sec:interactivity}
% to keep the discussion centered around future challenges and our vision
% on dataframe optimization with respect to the operator semantics.
% Specifically, the semantics of \code{GROUPBY} in \pandas are
% different than the traditional \code{GROUPBY} in relational algebra,
% but those semantics can be expressed in the algebra we presented.
% In \pandas, the semantics are a column-wise groupby followed
% by some operator. There is an intermediate object created by
% \code{df.groupby} calls in \pandas, which can be reused.
% }

\com{(A3) 
It would be nice to see more discussion
on the interplay between dataframes and data visualizations.
}

Visualization is indeed 
an important component
of data exploration with dataframes,
and not mentioning it was an oversight.
We now have added a brief 
discussion in Section~\ref{sec:interactivity} 
on how the default 
tabular view displayed when dataframes are printed
(a prefix/suffix of the rows and columns)
is a simple form of visualization for 
debugging and validation of structure and order,
but other forms of visualization may also be 
valuable.
We also have added a discussion around 
how prior work on approximate
decision making with visualization for
debugging and validation may be adapted.
% We then 
% focus our research questions around
% activities performed during data exploration,
% including visualization;
% one specific instance is how 
% approximate query processing (AQP) 
% can be applied to dataframes to 
% generate aggregate visualizations.


% \agp{Revise in a way that can highlight unique aspects to dataframes.}
% \done{
% Visualization is an important component of the dataframe data science
% life-cyle, and not including a discussion about this relationship
% was an unfortunate oversight. We have added a discussion in Section~\ref{sec:interactivity} on how dataframes are used with visualization and how they may be optimized in the future. Specifically, we argue how the tabular view is the one of the most common form of visualization of a dataframe. We also describe three class of optimizations for providing interactive feedback, so that users can quickly visualize and validate structural and order information of the dataframe. In addition, we also describe how approximate query processing (AQP) can be applied to dataframes to generate aggregate visualizations, citing prior work in this space.
% }


\com{(A4) 
The visonary aspects of the paper are dissappointing.
The authors discuss standard interactive data exploration tasks rather than
discussing the specific challenges posed and opportunities created 
as a result of dataframes.
}

We appreciate this comment, and have taken it to heart -- please see responses to
(M2/M3).


\com{(A5)
It is hard to print the PDF and, having gotten it printed,
the math symbols were not properly rendered.
}


We have re-rendered the Math symbols in the PDF to allow for easier printing.


\com{(A6)
It was surprising that there were no row-level schemas.
}

%\agp{This needs fixing based on joe's updates}
% \agp{We need two lines in the dataframe data model
% section about this.}
% \devin{We go into deep detail in this in Section 5, is that not enough?}
This is an interesting point!
Both the relational model and \pandas have schemas on only one axis: columns.
For relations, this is because of the distinct semantics of rows and columns.
Perhaps in \pandas this is because of the desire for a single default interpretation of a cell:
we always use the column type to interpret the bits in a cell. 
One could of course have an alternative row-based interpretation 
as you suggest, though. This is achieved in dataframe libraries like \pandas, as well
as our algebra, by applying a transpose operator (which of course is not in SQL!)
to shift interpretation.
However your observation is intriguing. We now highlight this point in Section~\ref{sec:dataframedef},
and discuss the resulting optimization challenges (i.e. the need to transpose
just to shift one's interpretation) in Section~\ref{sec:rowcolumneq}. 

% We opted for column-level schemas without row-level schemas 
% as is traditional in relations,
% as well as in \pandas via the \code{dtype} operator.
% We could have instead opted for row-level schemas 
% without column-level schemas
% wherein we apply our schema induction function on rows.
% In our formalism, we effectively 
% achieve this by transposing first,
% and treating the result column-wise.
% Our decision to opt for a single axis of schematization
% is so that 
% we have
% a unique interpretation for the value of each cell
% in the dataframe.
% That said, we could support schematization across both axes,
% and we discuss the performance implications
% for doing so in Section~\ref{sec:datamodel}.

% Indeed, we could have chosen to include row-level schemas.
% Row-level schemas or row typing, 
% for example, could be very useful
% if a dataframe has a fixed type across
% the rows but not the columns, so that
% on transposing it, we can recover the types correctly.
% Row typing is less useful (and adds a lot of unnecessary storage overhead) 
% when there is an array
% of types along a row, e.g., [<int>, <string>, <float>],
% as is likely when the column types are all distinct.
% Therefore, instead of forcing row typing in our model,
% we made it optional. 
% Implementations are free, however, to keep track
% of row-level schemas to avoid
% expensive schema induction after a transpose.
% We have added a discussion
% on these tradeoffs are a future research challenge
% in Section~\ref{sec:datamodel},
% and mention the fact that row-level schemas
% can be used in Section~\ref{sec:dataframedef}.





% \done{
% We have added a discussion on maintaining row-level schema in 
% Section~\ref{sec:datamodel}.
% We choose not to define row-level schemas as a part of the core data model,
% rather we allow it to be an extension that implementations
% can choose how to handle.
% We chose not to enable tuple types in the supported Domains
% to simplify the data model, and rows would be most specifically typed by a tuple
% containing each type of the columns. In practice, implementations are free to
% track and maintain a row-level schema if they choose, but it is not a
% requirement of the data model itself.
% A dataframe with heterogeneously typed columns will have rows that are
% tuple-typed. With a TRANSPOSE, the columns would become tuple typed.
% }

\com{(A7)
In the performance figure, why was there was a spike in variance around 100GB,
which was followed by a normalization of perofmance numbers.
}

After rerunning the experiments, we concluded that the spike in variance
was due to some contention in resources. We repeated the experiments additional times and did not see the variance spike in the
updated results. The new numbers are reported in 
Figure~\ref{fig:performance}.



\subsection*{Reviewer 2}
\com{(B1) 
The microbenchmarks do not demonstrate the strength of the underlying data model
as it's strength is in the assembly of the operators,
which does not occur in the microbenchmarks
}

Our goal with the microbenchmarks is to 
validate that simple optimizations (such as parallelism) 
within \modin 
can lead to substantial improvements
in scalability and performance over \pandas,
which has severe issues, despite being widely used.
To clarify this point further, we have moved
the \modin section to Section~\ref{sec:modin}
as opposed to Section 4 (in the previous version),
and focused more on lessons learned from our engineering
experience with \modin, and how that guides 
our future research directions. 
Indeed, further experiments to test the strength of
the underlying model and rewriting rules are needed, 
but we consider that as part of our future research agenda
and will do so in future work.



% The purpose of the microbenchmarks is to demonstrate that \modin gets
% considerable speedup over existing implementations with simple
% parallelism. It points out that despite having a lack of 
% scalability and performance, \pandas is extremely widely used.
% As a future work, we will add benchmarks demonstrating
% the strength of the algebra, however since this is a vision paper not
% focused on any specific implementation's performance, we would
% prefer to keep the current microbenchmarks simple as-is, so as not to distract
% from the central message of the paper.


\com{(B2) 
The paper, after the technical details of Modin,
is a grab bag of notes on existing work in databases and data science.
The discussion is somewhat direction-less and there is no true vision expressed here.
}
This feedback was addressed while resolving (M2/M3).
We have taken this feedback to heart and entirely revamped
Sections~\ref{sec:datamodel} and \ref{sec:interactivity} to be centered
on novel dataframe aspects. 


\com{(B3) 
Table of operator is not legible in printouts.
}


We have fixed the table to be more legible in printouts 
with a larger text size.


\com{(B4) 
Typo when discussion operators:
``... as well as four new operators.. We briefly describe... the three new operators.''
}


We have fixed this typo to describe the four new operators.


\com{(B5) 
It is unclear whether the types of values are represented and inspectable at run time.
}

Types are inspectable at runtime, and inspecting the types
will trigger their materialization if they are already not
materialized. We have added this clarification to 
Section~\ref{sec:datamodel}.
% \agp{Where is this? I don't see it. To me, it should be in Section~\ref{sec:definitions}, not in Section~\ref{sec:datamodel}.}
% \devin{
% We frame this as a challenge because it's really only accessible via 
% \code{GROUPBY} or \code{MAP}.
% Is this worth mentioning in \ref{sec:definitions}?
% }


\com{(B6) 
Some of the rewrites should be removed and 
be replaced with fewer but more in-depth rewrites.
}

We agree with the reviewer that the number of rewrites
in Section~\ref{sec:algebra-example}
was excessive and was not adding much to the discussion.
We have instead decided to focus on \code{pivot} as a single
case study---a challenging operator for relational algebra---and
described it in more detail with a new diagram.
% We have trimmed the number of rewriting examples in 
% Section~\ref{sec:algebra-example} and gone more in-depth about the
% pivot case, which is the most challenging case for relational algebra.
% The section has been rewritten to focus more generally on the display of
% the data model and less about any specific implementation.
% }

\com{(B7) 
The statement that ``query optimization is not possible in an eager system''
is misleading because most query optimization is performed before the evaluation of the program.
}

We were not clear in our writing 
and did not intend for this interpretation.
Dataframe systems, unlike relational databases,
support an incremental mode of composition of queries
where programmers can specify a \stmt 
composed of one or more operators at a time (i.e., a query sub-expression),
building on the variables declared in previous \stmts.
We revised Section~\ref{sec:interactivity}
to clarify that, by ``eager'',
we mean that the query processor executes each \stmt
as soon as it is invoked by the programmer, without waiting.
By ``lazy'', we mean that the query processor waits 
until the dataframe is either printed or saved before
it finds an optimized query execution plan that is 
semantically equivalent 
to executing each of the operators 
of query sequentially,
and executes this optimized query plan.
In this context, we believe that the ``eager'' mode
makes it difficult to perform query optimization
since the query processor will need to produce
results for each intermediate sub-expression as assembled by the user.
We have reworked this entire section and 
taken out the ``not possible'' part as it was confusing;
we have also added an example to illustrate this further.

% Thus, in this context, we believe that it is impossible to have
% efficient query plan when the query processor 
% naively and immediately executes
% each operator in the order that the programmer 
% calls them in the statement.
% \agp{agp to review}

\com{(B8)
The idea that lazy query processors ``recently emerged'' is flawed
as the on-demand evaluation of complex algebraic plans (e.g., Volcano)
has been the default mode of execution in query processors for decades.
}

We were not clear in our writing when stating that 
``the lazy paradigm ... recently emerged.''
We revised our submission to make it clear that
we are discussing eager and lazy evaluation
in the context of other dataframe and dataframe-like systems 
such as Pandas, Dask, and Spark, 
and not in relational databases 
which do not have
an incremental mode of composition.
In the context of dataframe systems,
eager execution, as described in the previous point,
is the canonical approach as is the approach used
in dataframe systems up until recently (e.g., Pandas and R Dataframes).
It is only recently with Spark dataframes and Dask 
have dataframe or dataframe-like 
systems begun operating within a lazy paradigm.
But since this point is subtle, we removed
any mention of whether the emergence was recent, 
and focus more on conveying the two modes as is,
centered on dataframe and dataframe-like systems.
% \agp{agp to review}
% \devin{I took out the whole ``recently emerged'' argument. It added nothing and served as a distraction.}

\com{(B9)
There should be more discussion around multi-query optimization and materialization.
Particularly, there should be more discussion on how the system would
predict which intermediate results would be more likely to be used.
What information would be necessary to drive such inferences?
}

% \agp{I don't believe we have added any discussion on this to the paper AFAIK.
% We should be talking about statistics that can help drive prediction.}
We have added further discussion on materialization and reusing
query results to Section~\ref{sec:interactivity},
taking advantage of ample user think-time. Specifically,
we discuss the need to predict user intent based on past workloads~\cite{ucsd-dataframe-study}
and operator lineage. We discuss the challenges in materialization
of intermediate results given that we may have many query fragments
partially completed. 
We also propose interesting future work on
embedding materialization decisions within the opportunistic
evaluation query planner to further accelerate the interactive user experience with speculative execution.
% We also discuss some interesting future work in
% integrating a materialization decision engine with the opportunistic
% evaluation approach to interactive query planning to enable
% some speculative execution as a part of the query plan for even
% faster results for the interactive user.
% \agp{At least a couple more sentences that start with "Specifically, we ..." }

\com{(B10)
It may be hard to do prefix computation when considering more complex expressions
as the system may need more than k rows to be able to display a prefix of size k
after more operations have been added to the expression.
What is the approach that Modin will take to this issue?
}

% \agp{I don't think this is our approach to answering this question. We
% are describing novel aspects wrt prefixes and order. Need to discuss.}
% \done{
% Because prefix computation with complex expressions is not a challenge that is
% specific to dataframes, we chose not to focus on it to place a higher importance
% on dataframe-specific challenges.
% }
% \devin{This needs to be updated if it is not already}
We have added a deeper discussion in Section~\ref{sec:datamodel} 
on the novel aspects of prefix computation
and the challenges in preserving order 
with prefix computation. As the reviewer mentions, it is
not always possible to know how many
rows a given query will output, and keeping aside
only $k$ rows will not always work, especially in complex queries
with selective predicates---this question is not new to dataframe systems
but the ordering aspect is novel. 
One approach, for example, would be to use operators that generate
results in order, such as index nested loop joins,
which progressively ingest more of the input dataframes until 
$k$ output rows are produced.
We can also leverage parallelism to 
prioritize the ingest
and processing of ``enough'' of the inputs to guarantee
the output of the first $k$ rows.
Since dataframes
must {\em guarantee} both the top $k$ and its order,
that dataframe query optimizers may need to use both 
selectivity and cardinality estimates, along with
models of past user behavior to gain 
insight into how many
input rows may be necessary to generate $k$ output rows. 
% This research may yield
% some interesting results that can also be applied to
% RDBMSs.
% \agp{this is weak: we only say we will look at past history. need a better argument.
% will revisit after i read s6}

\com{(B11) 
Sections 5 and 6 should be more concrete and try to have a focused vision
that shows how the algebraic approach can be an advantage on the current
state-of-the-art (e.g., Pandas and R).
This may be the focus on query planning to defer or avoid costly
data restructuring operations or 
a reversal of roles of data data and meta-data.
}

\com{AND}

\com{(B12)
There should be a connection between the technical details described in the beginning
and the vision described in the rest of the paper.
It is ok if this makes the vision of the paper becomes specific to the Modin view of dataframes.
}

This feedback was addressed while resolving (M2/M3).
We thank the reviewer for the query planning points---we have used them 
when reframing our vision when centered around novel
aspects of dataframes.
We have also substantially revised the previous portions of the paper
to keep only as many technical details as is needed
to ground our discussion on the vision.

\subsection*{Reviewer 3}
\com{(C1) 
Please cut out a bunch of details, we don't need a 12 page vision paper.
\squishlist{}
    \item I don't really need a 1-page example on data frames.
    \item Why do I need to know the history of data frames?
    \item Perhaps we do not need the exact formalism for the data model and all operations and
    a detailed sketch would suffice.
\squishend{}
}

This was resolved while addressing (M1). We provide some additional
details below.

We thank the reviewer for these suggestions.
We retained the example, but substantially reduced its length
and detail as it allows database readers who are unfamiliar
with dataframes to establish a basic understanding.
We have also redrawn the figure to reduce the space taken for it.

We have reduced the length for the history of dataframes,
only emphasizing key background for the interested database reader.
Specifically, we retained the portions that 
contribute a meaningful and largely unknown piece 
of how dataframes
emerged to the scientific community. 
This background also 
gives a basis on which we can
understand how dataframes were intended to be used, 
so that we can optimize
them in this context.


Finally, we have substantially reduced the length 
and details 
in the formalism
for the data model and algebra, 
reduced the number of rewritings,
and removed the extensions. 
We focus on the
components which make dataframes difficult to scale. The formalism
is important because it provides a basis upon which we can build
our research vision---and we only retain as much as is needed
to support that. 
We have also clarified the intention of this section.

Given the overwhelming popularity of dataframes
and their important role in the data science ecosystem,
as well as the relative lack of awareness and understanding
from the database research community,
we believe that the length of this paper is justified.

% Given the overwhelming popularity of dataframes and their important position in the data analysis ecosystem, we believe that the length of this paper is commiserate with the urgency for the database community to seize on this historic opportunity to make its mark on the future of computing. 
%This warrants detailed and exhaustive introspection on future research directions. As such, we have added substantial content on concrete research opportunities spanning many relevant areas of databases research.


\com{(C2) 
Missing related work.
There should be explicit mention of embeddable DBMSs such as DuckDB and SQLite
and, at least, a theoretical comparison of them and the vision proposed in the paper.
Also, please cite Tukey's book on EDA.
}

Regarding embeddable DBMSs, from an architecture perspective, we now 
clarify in Section~\ref{sec:modin} that Modin is a library, much like an embeddable DBMS. (This is standard for 
dataframe libraries, including pandas, so we overlooked mentioning it in this environment. It's a nice
connection to make, thanks!) In Section~\ref{sec:flexschemas} we also address some of the implications that arise 
for dataframes from having their storage external to the application, including some of the work in the 
community (e.g. Apache Feather) to address this. Finally, with respect to theoretical issues, the bulk of the 
paper focuses on distinctions (both theory and practice) that arise from the semantic distinctions
between relational databases (embedded or otherwise) and dataframes, so we hope there's sufficient discussion
of DBMSs vs. dataframes in general.

% \jmh{Why fight? I vote to skip this}
% Our entire thesis is that
% we must design dataframe systems from the ground up to support
% the unique characteristics of dataframes, including 
% flexible schema/dynamic typing,
% data-metadata and row-column equivalence,
% centrality of order, and differences in algebraic operators.
% Thus, any system whose interface is SQL-like and whose data model
% is relational is not a good fit, including embeddable databases.




% While embeddable DBMS systems could be a possible candidate
% for a processing and storage engine for dataframes, 
% given the vast differences
% in characteristics, including flexible schema/dynamic typing,
% data-metadata and row-column equivalence,
% centrality of order, and differences in algebraic operators,
% we do not believe it would be a good fit---and instead believe an
% approach that takes these characteristics as first-class citizens
% as opposed to bolting them on post-hoc, would
% be much more efficient and scalable.
% \agp{I think the following line should be dropped.
% Instead, we can replace it with one line around how the goals
% and vision are very different.
% Perhaps they may be satisfied if we add a line that says 
% that we can use an embeddable DBMS 
% as a storage/processing layer for dataframes?}
% We did not included the comparison of embeddable DBMS and dataframe as we believe that the scope of these systems are somewhat tangential, so we have limited this discussion to keep the dataframe vision the central point of the paper.

% We have clarified the related work section, Section~\ref{sec:}
% and
% The theoretical comparison to the data model was expanded upon
% and clarified, but to keep the vision the central point of the paper
% we have limited this discussion.
With respect to Tukey, we are big fans, and have happily added a citation to Tukey's book in the introduction.
Thanks for pointing that out -- sometimes we take our heroes for granted!

\com{(C3) 
The future vision is a bit generic.
Although sections 5-7 are the more interesting parts
with a particular emphasis on section 6,
they are only 2 pages out of the entire paper.
These sections should have a higher fraction of the paper
by adding more depth to the challenges and future directions
and making them less generic would also help.
}

This feedback was addressed while resolving (M2/M3).
We have taken this feedback to heart and have substantially revised
the vision portions of this paper.



==> old_opt.tex <==
\subsection{Workflow-based optimization}
\stitle{Deferred computation}
% - metadata expire/maintenance (only when recs not fresh)
% - lazy regeneration of vis only upon print 
During an analysis session, users constantly modify and operate on dataframes, which means that the metadata and associated recommendations can change quite significantly throughout a session, especially during reshape and type-modifying operations. This means that unlike in conventional visual analytics interfaces, where metadata can simply be computed once upon initial loading and assumed to stay fixed throughout, metadata needs to be constantly maintained to ensure that recommendations are generated correctly. As a result, the metadata computation associated with keeping the metadata always ``fresh'' after each dataframe operation can incur a high cost.
\par Our key observation was that since users often interspersed dataframe printing with a several dataframe operations, there is a high chance that the computed metadata and recommendations would be outdated again before the users has a chance to even see the results (as shown in Figure~\ref{fig:workflow}). As a result, we can delay the metadata computation and recommendation generation and compute only after a user has explicitly printed out a dataframe. Each \luxdf keeps track of how ``fresh'' the metadata and expires them when an operation performs in-place modifications, columnar access and updates, and value updates. Additionally, the recommendations are also expired when the intent is modified. Upon printing the dataframe, Lux recomputes the metadata right before the Compile stage in intent processing and generates the recommendations accordingly. This lazy evaluation strategy ensures that there is zero overhead on any dataframe operations. Currently, \lux currently expires metadata upon any write-based operations. Future work on a more intelligent, fine-grained maintenance of metadata can improve system performance (e.g., only refresh metadata for column X instead of entire dataframe when \texttt{df["X"]= ...}).
\stitle{Memoize repeated computation}
% - smart caching; (when print twice)
\lux memoizes the metadata and recommendations so that when any subsequent prints to the dataframe does not require recomputation in cases where the metadata and recommendations are not expired. This can happen in cases when the dataframe is printed twice without any modifying operations in between. While this may sound like an overly specific use case, such operations are in fact very common in exploratory workloads. In dataframe sessions, users more commonly perform ``non-committal'' operations that generate new dataframe or derived object for quick experimentation on the dataframe. As shown in In[3-5] in Figure~\ref{fig:workflow}, users may try to print out a column, perform grouping and aggregation, or print out descriptive summaries, all without modifying the base dataframe. In this case, when the user revisits the original dataframe, the memoized recommendations are immediately accessible to them.
\begin{figure}[h!]
    \includegraphics[width=\linewidth]{fig/workflow.pdf}
    \caption{Use case example demonstrating the applicability of workflow-based optimizations}
    \label{fig:workflow}
\end{figure}
\subsection{Visualization-based optimization}
In addition to the workflow-based visualizations, \lux applies a set of optimizations to speed up visualization processing and rendering. \lux applies random sampling when there are more than 30k rows in the dataframe \lux samples the dataframe down to a cap of 30k points, when there are more than 10k rows \lux samples 75\% of the datapoints. The selection of these cutoff parameters are selected based on settings that would lead to interactive responses. Users have the ability to tune these parameters, or turn off sampling completely and perform their own sampling on the dataframe externally.
\par For interactive visualizations in Vega-Lite, our preliminary experiments show that the majority of time was incurred on the frontend for rendering scatterplots. Following best-practices from visualization literature~\cite{Wickham2013BinsummarisesmoothA}, we applied binning techniques to display binned heatmap in place of scatterplots when the number of rows exceeds 5000. While the binned heatmap is better at alleviating the overplotting problem in scatterplots, the binning makes it more difficult to exactly locate the datapoints that lies in each bin.
%visualization-based optimizations can result in a loss of ---- 
% \stitle{Sampling}
%     - Vis-specific: sampling
% \stitle{Binned heatmap}
%     - scatterplot heatmap 

\doris{Several limitation for our current implementation: 1) limited sharing across different visualizations, 2) currently some optimizations are tied to the executor themselves (binning, sampling), while some are separated from the executor (metadata maintenance + caching).}


==> rebuttal.tex <==
%!TEX root = main.tex

% \begin{center}
\noindent {\large \bf Summary for Revised Paper \#75 ``Lux: Always-on Visualization Recommendations for Exploratory Dataframe Workflows''}
% \end{center}

We thank the reviewers and meta-reviewer for their detailed 
and insightful feedback, for answering additional questions during the revision period, and for giving us the opportunity 
to address their feedback in a revision.  
We have prepared a new version of the paper based on their suggestions, 
with updates to every section. We believe that the paper is much stronger as a result.

In brief, the changes made include:

\smallskip
\noindent {\bf \em A. Revised section outlining technical contributions (\cref{sec:intro}).} 
We have rewritten a lot of the introduction to better highlight our technical contributions. Specifically, we removed descriptive content that was unrelated to the contributions. Additionally, we identified the novelty of our work in each section, from the dataframe interaction framework (\cref{sec:framework}), to the intent language (\cref{sec:intent}), to recommendations (\cref{sec:rec}). We have also elaborated on how our performance optimizations builds on prior work in approximate query processing~\cite{GarofalakisG01, CormodeGHJ12}, early pruning~\cite{fastmatch}, materialization and reuse~\cite{GuptaM05, TangSEKF19}, and asynchronous computation~\cite{Xin2021,BendreWMCP19}. 

\noindent {\bf \em B. Revised sections comparing \lux with existing approaches (\cref{sec:relatedwork},\cref{sec:intent}).} 
The reviewers and metareviewer requested a fair comparison with visualization recommendation systems like Draco and a discussion on where the technical boundaries lie. We added two new related work subsections (in \cref{sec:relatedwork}) introducing existing approaches in visualization recommendation and specification, to provide background for the discussion. Moreover, we have substantially rewritten the intent language section to compare the \lux intent language design with existing recommendation and specification approaches. Within this section, we added a new discussion subsection (\cref{sec:intent_design_consideration}) describing our design considerations focused around versatility and convenience. We demonstrate how our intent language supports quick and flexible programmatic specification.
%why versatility and convenience are important design considerations for the intent language.
% The entirety of this section was written to address the concerns of the Reviewers and Metareviewer.

\noindent {\bf \em C. New section on novel dataframe interaction (\cref{sec:framework}).} 
We have significantly redesigned the presentation of our dataframe interaction framework to contextualize how the new framework differs from existing visualization specification approaches. Specifically, we have added new Figure~\ref{fig:framework} to outline the differences. We also reworked the different layers in our multi-tiered framework to clarify the confusion around terminology raised by reviewers.

\noindent {\bf \em D. Revised section on post-deployment lessons and findings (\cref{sec:evaluation}).} 
To fit the theme of the SDS track, we added a completely new section around the implementation challenges, lessons learned, and post-deployment analysis. The lessons are distilled from needs and requests emerging from real-world usage of \lux in the open-source community. These post-deployment findings is a novel and unique strength of the paper intended to be instructive for future system-designers.

\noindent {\bf \em E. Other significant writing changes.} 
We have made considerable changes to the text 
of the paper to improve its overall readability. Specifically, we have focused on making the paper more clear, formal, and concise. 
To accomodate to the shortened page length in the SDS track, we have aggressively trimmed the introduction, system, and optimization descriptions. 
Unfortunately, due to the new additions and shortened page limit, 
we had to move some of our content, including the secondary performance experiments and first-use user study evaluation, to our extended technical report~\cite{lux-tr},
as we will describe below.
% We have also delegated the secondary performance experiments and first-use user study evaluation to the technical report.  

\smallskip
The changes in the paper are highlighted in \change{{\bf blue}}. We address the specific points raised in each of 
the individual reviews below, starting with the meta-review.


% \agp{Did we want to paste in the action items from email discussion with Juliana
% as well so that we make 
% sure we respond to those too?}\doris{see commented below, the summary of changes addresses each of these point by point.}
% - fair comparison with baselines in terms of recommendation. Specifically, a fair-effort attempt to encode intents into recommendation systems like Draco, and commenting on where the technical boundaries lay. This covers points 1 and 2 in the email
% - focus on the technical contribution. This should enable the authors to cut content that is unrelated to the contributions. In our opinion, the main contributions are the intent-based hints and integration into a Jupyter environment
% - Part of the evaluation can discuss “the design choices and implementation challenges, lessons learned, and post-deployment analysis”,

\subsection*{Metareview}
\com{(M1) Clearly state the novel technical contributions in the introduction. We note that points 1, 2, 4, 5 primarily describe what Lux does and how it works, rather than its novelty.}

We have rewritten and shorted the introduction to emphasize the novel technical contributions of our work. We have also substantially reworked our related work section (now Section~\ref{sec:relatedwork}) to emphasize the differences with respect to prior work. In addition, we have made the following changes to the body of the paper to delineate our key technical differences: 
\begin{denselist}
    \item In Section~\ref{sec:framework}, we reorganized our novel dataframe interaction framework and compared it with existing visualization specification workflows. 
    \item In Section~\ref{sec:intent}, we now highlight how the \lux intent language substantially differs from existing recommendation and specification approaches in that it enables flexible specification without an explicit focus on visualization creation. We also show how it requires fewer lines of code (new Figure~\ref{fig:comparison}) and how it is more versatile in supporting intent beyond explicit visualization creation.
    \item In Section~\ref{sec:rec}, we summarized the recommendation section to focus on the two novel classes of recommendation specific to dataframe workflows.
    \item In Section~\ref{sec:compute}, we outline the key differences between the optimizations applied in \lux as compared to existing techniques, described more in our response to M3.
\end{denselist}

\com{(M2) Directly acknowledge and compare with related works. Specifically Lux's recommendations and intents overlap with or could be expressed by Draco, Voyager, and Showme. The observable ecosystem is also related, and supports embedded interactive visualizations and recommendation systems.} 

Systems such as Show Me~\cite{Mackinlay2007}, Voyager~\cite{Wongsuphasawat2016,Wongsuphasawat2017}, and Draco~\cite{moritz2019formalizing} have proposed influential techniques that shape the discourse around visualization recommendation. The key difference between these systems and \lux is that these papers leverage perceptual effectiveness as a ranking criterion, whereas our work supports recommendation based on data interestingness and applies visualization best practices to generate recommendations. We have rewritten Section~\ref{sec:relatedwork} to elaborate the differences with respect to related work. Moreover, we highlight how our intent language is different from these existing approaches via a discussion and a new comparison figure in Section~\ref{sec:intent}.

\com{(M3) clearly distinguish the deltas from existing workflow and query optimization techniques such as lazy evaluation, view maintenance, AQP, streaming visualization.}

The optimizations in \lux extend standard database optimization techniques but leverages the unique problem requirements in dataframe workflows and visualization recommendations. We have included additional clarifications and citations in Section~\ref{sec:compute} to outline how we adapt existing techniques. For example, our \wflow optimization leverages existing work on caching and reuse~\cite{GuptaM05, TangSEKF19}, but identifies common usage patterns in a dataframe workflow to intelligently determine when the metadata and recommendations need to be recomputed.


\com{(M4) Update the paper to fit the SDS track}

We have drastically reduced the length of the paper to fit in the page limit of 10 pages. 
In addition to the clarifications and additions suggested by reviewers, we have made the following revisions to reduce the verbosity of the paper: 
\begin{denselist}
    \item \cref{sec:relatedwork}: Removed discussion around GUI and programming, including Wu et al.~\cite{B2} and Kery et al.~\cite{mage}, in favor of the added related work on visualization specification and recommendation.
    \item \cref{sec:framework}: Reduced the length of dataframe interaction framework to focus on the differences with respect to existing workflows.
    \item \cref{sec:rec}: Removed discussion of visualization recommendation techniques drawn from prior work (intent and metadata-based recommendations), focusing only on novel dataframe-specific recommendations introduced by \lux.
    \item \cref{sec:system}: Reduced the lengthy discussion around system components, including parser, validator, and compiler.
    \item \cref{sec:user}: Rewritten the user study to summarize lessons learned.
\end{denselist}

\com{(M5) Focus on the design choices and implementation challenges, lessons learned, and post-deployment analysis}

We have added a new subsection in Section~\ref{sec:evaluation} to summarize the implementation challenges, and lessons learned from our post-deployment evaluation. In brief, we describe the engineering challenges around metadata propagation, fallback options, and downstream exports.

\com{(M6) Data science is a broad term that goes beyond record-based visualizations. Please clearly state the paper’s scope up front.}

We agree with reviewer's comments around the broad term ``data science''. We have narrowed the scope of the paper by changing the title and rewriting the introduction to be more focused on exploratory dataframe-based workflows. 

\subsection*{Reviewer 1}
% \com{(A1) the novel aspects beyond the seamless integration of various (pre-existing) ideas into notebooks could be strengthened.} 
\com{(W1) I am conflicted concerning the presentation of the paper. It reads, to some extent, as an extended demo paper rather than a research paper. I even read the word demo at some point. As a system research paper, I suggest rebalancing the paper more towards technical content and novelty, which can be improved, I think.}

See our response to M1.

\com{(W2) I would have appreciated more depth in the discussion and evaluation of the novel types of recommendations and the efficient execution engine.}

We have now rewritten Section~\ref{sec:rec} to describe only the novel, dataframe-specific recommendations and have removed the description for the metadata and intent-based recommendation which were drawn from our prior work~\cite{frontier}. See our response to M3 for changes on the description of the execution engine.

\com{(W3) The evaluation does not consider a baseline approach, i.e., a classical workflow used today. This would I think strengthen the validation of the system's main advantages/ points to improve.}

In this paper, we adopted a realistic evaluation study to explore how data scientists make use of \lux in their existing workflow. We specifically asked open-ended questions about how the tool compares with existing workflows, such as the usage of Tableau and matplotlib. We have rewritten the user study the emphasize the differences with existing workflows. One inherent challenge with field studies of this sort is that the evaluation is largely qualitative and less amenable to a direct baseline comparison compared to a controlled lab study~\cite{Isenberg2008,Plaisant2004}. For example, we could have performed a lab study that compared \lux with a manual specification approach as a baseline, however, the artificial task and dataset setup would make it difficult to study how \lux truly fits into a data scientist's dataframe workflow. It is also unclear how to pick an appropriate metric for an exploratory setting with no explicit analysis goal~\cite{North2006}. We have added a note to outline this limitation in Section~\ref{sec:evaluation}.

% \com{(W3) In addition, some further details on the evaluation methods and scenarios involving more than one relation (as mentioned in the introduction) would be interesting.}

% See our response to Reviewer 1's D4.

\com{(D1) In Section 3.2.2, the example query 2 is said to compute an average. This is not clear from the code shown. I assume average would be a default function here. In this case, it may make sense to point that out.}

We have added a clarification to Query 2 (now Query 3) to state that average is the default function.

\com{(D2) Example Query 4 seems inconsistent - I do not understand why the axis is MilesPerGal given the descriptive text.}

We acknowledge that we made a mistake in the label for Query 4. We thank the reviewer for catching this, and have corrected this statement in the revision. 

\com{(D3) Concerning the recommendation part, I am wondering how many recommendations are generated (I understand top-k where k is predefined) and how the ranking of these is done. The text refers to some score for interestingness, but this part remained quite vague. The discussion focuses on ranking based on the visualization cost, which is certainly an interesting dimension to consider, but it appears further details are omitted.}

The number of visualizations recommended is set to k=15 by default and is a parameter that can be adjusted by users. We omitted this detail from the paper given that this is not a central focus of the paper. See our documentation for more detail: \url{https://lux-api.readthedocs.io/en/latest/source/reference/config.html#modify-sorting-and-ranking-in-recommendations}


\com{(D4) The evaluation in Section 7 relies on datasets with a single relation only, while the introductory example suggests more complex scenarios can be handled as well. I would expect an evaluation with scenarios including more than one relation, as this may potentially have a signifiant impact on the answers to RQ1 and give a broader scope to RQ2.}


% The join example highlighted in Section~\ref{sec:demo} is just one of many data cleaning and transformation operations supported by the \pandas API. Further evaluations and scenarios involving joins is out of the scope of this paper, but can be found in example notebooks on our tutorials page: \url{https://lux-api.readthedocs.io/en/latest/source/reference/gallery.html}.
% % do not believe that this is central

The join example highlighted in Section~\ref{sec:demo} is just one of many data cleaning and transformation operations supported by the \pandas API. For the performance overhead reported in Table~\ref{tbl:workload}, \lux adds overheads after the dataframe function computation is done. As a result, the overhead does \textbf{not} depend on the time taken for the dataframe function computation itself. So two function calls, one being a join, and another being a filter, both resulting in the same dataframe, would lead to the same \lux overhead as long as the size/shape of the resulting dataframe is the same. So we believe our evaluation, by considering various sizes/shapes for the dataframes being operated on, does consider all possible dataframe functions implicitly, including joins.

\com{(D5) Concerning RQ3 listed in Section 7, the methodology remains somewhat unclear. How was a ground truth obtained? How do you validate that the recommendations are indeed interesting from a user perspective?}

The secondary experiment addressing RQ3 has now been moved to the technical report~\cite{lux-tr}. The ground truth ranking was determined by running \lux without the \prune approximation. This serves as a comparison of how the recommendation accuracy varies for different fractional sizes of the dataframe to be used in the sample. For the performance experiment, our goal is not necessarily to validate that the recommendations are interesting from a user perspective; the ranking is largely based on established interestingness metrics used in the visualization recommendation literature~\cite{frontier,demiralp2017foresight}.

\com{(D6) Runtime overhead appears to be a bottleneck looking at the graphs in Section 7, but this is not pointed out in the discussion. In my understanding, the overhead in Table 2 relates to the overhead for printing data frames (Figure 10). However, from Figure 9, I conclude that the average runtime of a notebook cell can go from less than 10 s for pandas to approximately 90 s with all optimizations. This makes me question the interactive performance.}

Figure~\ref{fig:macrobenchmark} shows the average runtime across all different types of cells in the notebook. As a result, it does not distinguish between whether a cell involves a print or non-print operation. Based on the numbers reported in Table 2, the overhead in the largest dataframe size that we have tested is less than 25 seconds. Given that the execution backend for \lux is \pandas, there are inherent scalability bottlenecks associated with \pandas as the data processing framework~\cite{modin-vision}. While this is not truly interactive (following the sub-500ms definition in Liu et al.~\cite{Liu2014}), our optimizations have still proven to yield orders of magnitude improvement on a vanilla implementation of always-on visualization display. In general, \lux is interactive for situations where working with \pandas is interactive (e.g., adding two seconds of overhead on top of medium-to-large real-world datasets). Moreover, our \async optimization ensures that the table view is displayed in a non-blocking manner, so that users are guaranteed a result even in the non-interactive scenario.

% For example, maybe saying that for settings where pandas is interactive, we are also interactive; for settings where pandas isn't interactive, we are also non-interactive? Or can we justify based on how large typical dataset sizes are on average that the non-interactive cases are unlikely? Can we also possibly say that we can support users in settings where Lux is non-interactive but pandas is by showing them the pandas results first before the toggle button shows up for Lux? Thereby giving them the best of both worlds? Irrespective the blurb feels a bit weak right now.
\subsection*{Reviewer 2}
\com{(B1) There are other existing systems for visualization recommendations that do not appear to have been compared against. To be specific about it, I do not think that relegating a discussion of Draco (reference 44 in the submission) to a single sentence in Section 9 is a sufficient dismissal given the many important similarities.}

See our response for M2.

\com{(B2) I found myself wishing for a more thorough study of the quality of the recommended visualizations, especially given the writing focus on the first sections of the paper on ``always-on recommendations''.}

Past studies have shown that recommendation accuracy is not the most appropriate metric to measure for evaluating visualization recommendations; instead, systems should offer a holistic yet interpretable set of categories~\cite{frontier,Zehrung2021}. The core contribution of the paper is the always-on framework, which is an extensible framework that adapts to any type of recommendation shown. This technique itself is not tied to accuracy, so we believe it would not be appropriate to measure its effectiveness that way. A user study that compares between visualization recommendations and manual exploration of data has been performed in Cui et al.~\cite{datasite} and Wongsuphasawat et al.~\cite{Wongsuphasawat2017}, and is outside of the scope of the paper. We note that our evaluation does qualitatively compare against other common visualization tools, including Tableau~\cite{tableau} and matplotlib~\cite{matplotlib}.

\com{(B3) The chosen word ``view'' to describe one of the layers of the system's architecture is confusing; the paper talks about ``dataframe evolution'' and ``view update'' and it makes me think of database views.}

We have renamed ``view'' to ``visualization'' in our dataframe interaction framework to avoid this confusion. Furthermore, we have reorganized the framework via the new Figure~\ref{fig:framework} to clearly demarcate the differences across the different layers.


\subsection*{Reviewer 3}

% \com{(C1) the technical depth and experimentation for each delta is not deep enough...the paper would be a much better fit for the industrial or data science tracks}

% See our response to M4.

\com{(W1, D1) The focus on dataframes only is in disconnect with the overall claim of ``Recommendations for Exploratory Data Science''.}

See our response to M6.

\com{(W2, D2) The focus on generating static visualizations seems limiting. Interactive visualizations have been shown to be more meaningful for exploration of multidimensional datasets.}

\lux's framework supports the level of interactivity enabled by the rendering system, but interactivity is not the focus of this paper. For example, visualizations in \lux are generated using Vega-Lite~\cite{satyanarayan2017vega}, which supports sensible defaults for interactive visualizations, such as hover tooltips, zooming, and panning all automatically out of the box. 

\com{(W3, D3) Main points of recommendation for data exploration is to allow users get to meaningful results and insights fast. The current studies, however, do not seem to quantify if the proposed tool helped interviewees reach to results faster or whether they managed to gain more insights in comparison to not having Lux.}

Prior work has already demonstrated the benefits of visualization recommendations in supporting exploratory analysis~\cite{datasite,Wongsuphasawat2016,Wongsuphasawat2017}. Insights are  notoriously hard to measure and evaluate, especially given the variability across use cases~\cite{North2006}. Instead our evaluation centers on qualitative differences between \lux and present-day workflows. By talking to \lux adopters in the open-source community, we can understand how \lux is being used in their workflows and why they have adopted it. 


\com{(W4, D4) The technical presentation and the discussion on experiments can be improved.}

We have significantly rewritten the experiments and user study sections to focus on the summary findings. 
For the evaluation study, we have now focused our discussion on the first experiment around the overall workflow performance, and deferred the detailed experiment on the effect of dataframe width and recommendation accuracy to the technical report~\cite{lux-tr}. For the user study section, we focused our discussion on the field study interviews and aggressively reduced the length of the discussion.

% \com{(D4) The current discussion in the experiments and user studies is dense, to the extent that useful insights are hidden. It would be more meaningful to include takeaway paragraphs to summarize findings.} 
% See our response to W4.

%Note that reviewers missed a D5 in their rebuttal
\com{(D6) The choice of k=15 for Recall@k seems arbitrarily large. (As recall@all=1, it would be more meaningful to show recall@k while increasing k.}

For the experiment, we chose the $k$ value to reflect the default setting in \lux to display the top 15 results in each action. This precision and recall experiment has been moved to the technical report~\cite{lux-tr}, since it is not central to the story of the paper.

\com{(D7) In Fig.9 it is unclear why adding prune to wflow is actually increasing overhead in some of the Communities experiments.}

For the experiments under $10^4$ rows, it is expected that the \prune + \wflow combination will perform worse than simply \prune. This is because \prune applies a sampling approximation only when the number of rows exceeds 30k (i.e., the minimum threshold for approximation to apply); as a result, \prune only yields benefits for the $10^5$ row trial for \communities. Comparing the effects of \prune on \airbnb and \communities ($\geq$10k), we note that the performance speedup from \prune for \communities is larger than that for \airbnb. This is because \airbnb contains a lower number of columns and lower cardinality columns and therefore the search space for most actions is fairly small. As a result, the \prune optimization is only applicable for Correlation and Enhance in \airbnb where the search space is large enough. On the other hand, given the large number of columns in \communities, the \prune optimization is applicable to all actions, leading to more savings from approximation over the recomputation cost.% (as described in Equation \ref{eq:prune_condition}).

\com{(D8) ``When compared against the baseline, Lux is over 100X faster for 100k Airbnb and over 650X faster for 10M Communities.'' Shouldn't this be the other way around?}

We acknowledge that we had mistakenly swapped the number of rows for the \airbnb and \communities datasets. We thank the reviewer for catching this, and have corrected this statement in the revision. 


==> terminology.tex <==
\subsection{Terminology}
Here we introduce the terminology associated with each level of interacting with dataframes as implemented in the Lux system. 
\stitle{LuxDataFrame} is the centerpiece of what the user interacts with in a visual dataframe workflow. The \luxdf acts as a wrapper around \pandas DataFrames, which supports all existing \pandas operations, while storing additional information regarding the metadata, structure, and history for generating visual recommendations. When Lux is imported, \luxdf dynamically overrides all new instances of Pandas dataframes via ``monkey-patching''~\footnote{\url{https://en.wikipedia.org/wiki/Monkey_patch}}, so that users can interact with the \luxdf as-if it is a Pandas dataframe.% \tr{Additionally, we provide \pandas-consistent output behavior by safeguarding \lux with informative warnings, falling back to \pandas upon internal erros, and providing the \pandas table as the default display.} %, so that the resulting view from \lux is at least as good as what \pandas would provide. %the notion of a \luxdf is largely hidden from an end-user's perspective. U
\stitle{Intent} is a set of description indicating what the user is interested in within a dataframe. When an intent is attached to a dataframe, the visualization based on the user-specified intent (i.e., \textit{Current Visualization}) is updated. The intent is used to generate groups of recommendations that are relevant to the Current Visualization. %When no intent is specified, a set of default recommendations are generated.%Lux determines the set of appropriate recommendations to display. The intent is used to update 
\stitle{Action} describes a set of visualization recommendation based on a specified search space and optionally ranks visualizations based on a scoring mechanism. \tr{For example, the \texttt{Correlation} action searches over a list of visualizations corresponding to all possible pairs of quantitative attributes and ranks each visualization based on the Pearson's correlation score.}
\stitle{VisList/Vis} corresponds to Views in Figure~\ref{fig:framework}. A \vis represents an individual visualization displayed in \lux. 
A \vislist represents collections of visualizations in \lux, which can either be constructed via an intent, or as a list of individually constructed \vis objects.
